Directed random walks on polytopes with few facets

Let $P$ be a simple polytope with $n-d = 2$, where $d$ is the dimension and $n$ is the number of facets. The graph of such a polytope is also called a grid. It is known that the directed random walk along the edges of $P$ terminates after $O(\log^2 n)$ steps, if the edges are oriented in a (pseudo-)linear fashion. We prove that the same bound holds for the more general unique sink orientations.

==> macros.pub.tex <==
\makeatletter

% This command, \reallynopagebreak, allows not to have a pagebreak between a
% list environment and the words preceeding it.
    {\gdef\reallynopagebreak{\par\nopagebreak\@nobreaktrue}}

%%% Font styles

\addtokomafont{sectioning}{\rmfamily}
\newcommand{\mathsc}[1]{\text{\textsc{#1}}}

\newcommand{\TODO}[1]{\textcolor{red}{[\textsc{Todo:} #1}]}

%%% New commands for math mode

\newcommand{\fin}[1]{{[#1]}}
\newcommand{\sink}{{\mathrm{sink}}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\one}{\mathbbm{1}}
\newcommand{\T}{\mathrm{T}}
\newcommand{\USO}{\mathrm{USO}}
\newcommand{\Sym}{\mathfrak{S}}
\DeclareMathOperator{\E}{E}
\newcommand{\from}{\leftarrow}
\newcommand{\From}{\longleftarrow}
\newcommand{\To}{\longrightarrow}
\newcommand{\given}{\;\big|\;}
\newcommand{\Ev}{\mathcal{E}}
\newcommand{\pivot}{\mathrm{pivot}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\Harm}{\mathrm{H}}

\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}

% A dot that is fatter than a \cdot, but not as fat as a \bullet.
% Needs the graphicx package.
\newcommand*\Cdot{\mathpalette\Cdot@{.5}}
\newcommand*\Cdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}


%%% Theorems and proofs

\theoremseparator{.}
\theoremheaderfont{\itshape}
\theorembodyfont{\normalfont}
\theoremsymbol{{\tiny\ensuremath{\blacksquare}}}
\newtheorem*{proof}{Proof}

\theoremsymbol{}
\theoremheaderfont{\bfseries\upshape}

\makeatletter
\let\nobreakitem\item
\let\@nobreakitem\@item
\patchcmd{\nobreakitem}{\@item}{\@nobreakitem}{}{}
\patchcmd{\nobreakitem}{\@item}{\@nobreakitem}{}{}
\patchcmd{\@nobreakitem}{\@itempenalty}{\@M}{}{}
\patchcmd{\@xthm}{\ignorespaces}{\nobreak\ignorespaces}{}{}
\patchcmd{\@ythm}{\ignorespaces}{\nobreak\ignorespaces}{}{}
\renewtheoremstyle{break}%
  {\item{\theorem@headerfont
          ##1\ ##2\theorem@separator}\hskip\labelsep}%
  {\item{\theorem@headerfont
      ##1\ ##2\ (##3)\theorem@separator}\hskip\labelsep}
\makeatother
\theoremstyle{break}


\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{observation}{Observation}
\newtheorem{conjecture}{Conjecture}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}

\theorembodyfont{\rmfamily}
\newtheorem*{definition}{Definition}
\newtheorem*{notation}{Notation}

\makeatother

